Learning an Artificial Language for Knowledge-Sharing in Multilingual Translation

The cornerstone of multilingual neural translation is shared representations across languages. Given the theoretically infinite representation power of neural networks, semantically identical sentences are likely represented differently. While representing sentences in the continuous latent space ensures expressiveness, it introduces the risk of capturing of irrelevant features which hinders the learning of a common representation. In this work, we discretize the encoder output latent space of multilingual models by assigning encoder states to entries in a codebook, which in effect represents source sentences in a new artificial language. This discretization process not only offers a new way to interpret the otherwise black-box model representations, but, more importantly, gives potential for increasing robustness in unseen testing conditions. We validate our approach on large-scale experiments with realistic data volumes and domains. When tested in zero-shot conditions, our approach is competitive with two strong alternatives from the literature. We also use the learned artificial language to analyze model behavior, and discover that using a similar bridge language increases knowledge-sharing among the remaining languages.

==> tables/manual_inspection.tex <==
\renewcommand{\_}{{\fontfamily{ptm}\selectfont\textunderscore}}
\begin{table*}[ht]
\tiny
\centering
\setlength\tabcolsep{1pt} % default value: 6pt
\begin{tabular}{ llllllllllllllllllllllllllllllllll } 
\toprule
\multicolumn{10}{l}{\textbf{From English-centric system:}} \\
English &  
\texttt{\textunderscore"} & 
\texttt{We} & 
\texttt{\textunderscore now} &
\texttt{\textunderscore have} & 
\texttt{\textunderscore4-} &    
\texttt{month} & 
\texttt{-} &        
\texttt{old} &    
\texttt{\textunderscore m} &     
\texttt{ice}  &   
\texttt{\textunderscore that} &  
\texttt{\textunderscore are}  &  
\texttt{\textunderscore non}  &  
\texttt{-} &      
\texttt{dia}     &
\texttt{bet}     &
\texttt{ic}      &
\texttt{\textunderscore that}  &
\texttt{\textunderscore used}  & 
\texttt{\textunderscore to}    & 
\texttt{\textunderscore be}    & 
\texttt{\textunderscore diabet} &
\texttt{ic}      &
\texttt{,"}      &
\texttt{\textunderscore he} &
\texttt{\textunderscore added} 
\texttt{.} \\
slice 1&
8224 &
4026 &
6163 &
3366 &
7883 &
6830 &
2552 &
5086 &
7962 &
2552 &
1489 &
2552 &
7159 &
2552 &
600 &
3296 &
2552 &
2552 &
6525 &
2552 &
3089 &
8549 &
2552 &
2537 &
3613 &
2622 &
6742 \\
slice 2& 
7334&
6626&
1893&
6055&
9048&
6691&
7043&
1355&
7671&
7043&
570&
7043&
4018&
7043&
7957&
3480&
7043&
7043&
3410&
7043&
2014&
99&
7043&
7517&
3064&
1580&
9808\\
Malay &
\texttt{\textunderscore ▁“}&
\texttt{\textunderscore Kami}&
\texttt{\textunderscore ▁kini}&
\texttt{\textunderscore ▁mempunyai}&
\texttt{\textunderscore ▁seekor}&
\texttt{\textunderscore ▁anak}&
\texttt{\textunderscore ▁tik}&
\texttt{\textunderscore us}&
\texttt{\textunderscore ▁yang}&
\texttt{\textunderscore ▁berusia}&
\texttt{\textunderscore ▁4}&
\texttt{\textunderscore ▁bulan}&
\texttt{\textunderscore ▁yang}&
\texttt{\textunderscore ▁sudah}&
\texttt{\textunderscore ▁tidak}&
\texttt{\textunderscore ▁menghid}&
\texttt{\textunderscore ap}&
\texttt{\textunderscore ▁diabetes}&
\texttt{\textunderscore ,”}&
\texttt{\textunderscore ▁beliau}&
\texttt{\textunderscore ▁menambah}&
\texttt{\textunderscore .}\\
slice 1 &
6134&
4026&
6163&
3366&
2552&
8852&
86&
2552&
2552&
3526&
7883&
6830&
2552&
8419&
5288&
7838&
2552&
9633&
2537&
3613&
2622&
6742\\
slice 2 & 
7334&
4360&
1893&
6055&
7043&
3518&
4612&
7043&
7043&
9169&
2909&
8806&
7043&
8482&
3410&
473&
7043&
5998&
2806&
3064&
1580&
9808 \\
\midrule
\multicolumn{10}{l}{\textbf{From Indonesian-centric system:}} \\
Indonesian &
\texttt{\textunderscore ▁“}&
\texttt{\textunderscore Sa}&
\texttt{\textunderscore at}&
\texttt{\textunderscore ▁ini}&
\texttt{\textunderscore ▁ada}&
\texttt{\textunderscore ▁menc}&
\texttt{\textunderscore it}&
\texttt{\textunderscore ▁umur}&
\texttt{\textunderscore ▁4}&
\texttt{\textunderscore ▁bulan}&
\texttt{\textunderscore ▁nond}&
\texttt{\textunderscore ia}&
\texttt{\textunderscore betes}&
\texttt{\textunderscore ▁yang}&
\texttt{\textunderscore ▁dul}&
\texttt{\textunderscore unya}&
\texttt{\textunderscore ▁diabetes}&
\texttt{\textunderscore ,”}&
\texttt{\textunderscore ▁tamb}&
\texttt{\textunderscore ahnya}&
\texttt{\textunderscore .}\\
slice 1 &
2502&
2502&
2502&
2502&
2502&
4083&
2502&
6798&
2821&
4083&
70&
2502&
7823&
2502&
6064&
2502&
9633&
2537&
6461&
2552&
6852\\
slice 2 &
7043&
8446&
8446&
1493&
8446&
5117&
8446&
6749&
1892&
8446&
8446&
8446&
3093&
8446&
8446&
8446&
3079&
7043&
8001&
8446&
4553 \\
Malay &
\texttt{\textunderscore ▁“}&
\texttt{\textunderscore Kami}&
\texttt{\textunderscore ▁kini}&
\texttt{\textunderscore ▁mempunyai}&
\texttt{\textunderscore ▁seekor}&
\texttt{\textunderscore ▁anak}&
\texttt{\textunderscore ▁tik}&
\texttt{\textunderscore us}&
\texttt{\textunderscore ▁yang}&
\texttt{\textunderscore ▁berusia}&
\texttt{\textunderscore ▁4}&
\texttt{\textunderscore ▁bulan}&
\texttt{\textunderscore ▁yang}&
\texttt{\textunderscore ▁sudah}&
\texttt{\textunderscore ▁tidak}&
\texttt{\textunderscore ▁menghid}&
\texttt{\textunderscore ap}&
\texttt{\textunderscore ▁diabetes}&
\texttt{\textunderscore ,”}&
\texttt{\textunderscore ▁beliau}&
\texttt{\textunderscore ▁menambah} &
\texttt{\textunderscore .} \\
slice 1 &
2502&
2502&
2502&
6953&
2502&
8857&
7838&
2502&
2502&
3526&
2821&
4083&
2502&
4083&
2821&
2502&
2502&
7838&
2537&
2552&
2537&
6852 \\
slice 2&
7043&
4360&
1493&
1933&
8446&
3253&
3261&
8446&
8446&
9169&
280&
8446&
8446&
8446&
8446&
7563&
8446&
3079&
5251&
8446&
5072&
4553\\
\bottomrule
\end{tabular}
\caption{
\label{tab:example} Example.
}
\end{table*}

